Recent Advances in Practical Data Reduction

Over the last two decades, significant advances have been made in the design and analysis of fixed-parameter algorithms for a wide variety of graph-theoretic problems. This has resulted in an algorithmic toolbox that is by now well-established. However, these theoretical algorithmic ideas have received very little attention from the practical perspective. We survey recent trends in data reduction engineering results for selected problems. Moreover, we describe concrete techniques that may be useful for future implementations in the area and give open problems and research questions.

==> chapter/frontmatter.tex <==
\sppTitle
  %[A Much Shorter Running Title] % <- This is optional
  {Recent Advances in Practical Data Reduction} % <- This is required

\sppAuthor{Faisal N. Abu-Khzam}{Lebanese American University, Lebanon}{faisal.abukhzam@lau.edu.lb}
\sppAuthor{Sebastian Lamm}{Karlsruhe Institute of Technologie, Germany}{sebastian.lamm@kit.edu}
\sppAuthor{Matthias Mnich}{Hamburg University of Technology, Institute for Algorithms and Complexity, Hamburg, Germany}{matthias.mnich@tuhh.de}
\sppAuthor{Alexander Noe}{University of Vienna, Austria}{alexander.noe@univie.ac.at}
\sppAuthor{Christian Schulz}{Heidelberg University, Germany}{christian.schulz@informatik.uni-heidelberg.de}
\sppAuthor{Darren Strash}{Hamilton College, USA}{dstrash@hamilton.edu}

\sppAuthorRunning{Abu-Khzam\etal} % <- This is optional; use only if there are too many authors to be display in the header

\sppAbstract{
Over the last two decades, significant advances have been made in the design and analysis of fixed-parameter algorithms for a wide variety of graph-theoretic problems.  This has resulted in an algorithmic toolbox that is by now well-established.  However, these theoretical algorithmic ideas have received very little attention from the practical perspective.  We survey recent trends in data reduction engineering results for selected problems. Moreover, we describe concrete techniques that may be useful for future implementations in the area and  give open problems and research questions.
}

%\sppAbstractOnline{ % <- This is optional
  %A separate abstract for \url{www.SpringerLink.com} can be provided here!
%}


==> macros.tex <==
% DO NOT CHANGE THIS FILE

% Landau
\NewFunction{Oh}{\mathcal O}
\NewFunction{OhTil}{\tilde{\mathcal O}}
\NewFunction{oh}{o}
\NewFunction{lTheta}{\Theta}
\NewFunction{lOmega}{\Omega}
\NewFunction{lomega}{\omega}

% Stochastic
\NewFunction[Sqr]{prob}{\mathbb P}
\NewFunction[Sqr]{expv}{\mathbb E}
\NewFunction[Sqr]{var}{\texttt{Var}}

% Common Sets
\NewSymbol{sN}{\mathbb{N}}
\NewSymbol{sNpos}{\mathbb{N}_{>0}}
\NewSymbol{sZ}{\mathbb{Z}}
\NewSymbol{sR}{\mathbb{R}}
\NewSymbol{NP}{\mathcal{NP}}

% Abbreviations
\NewAbbr{etal}{~et~al.}
\NewAbbr{eg}{e.g.,}
\NewAbbr{cf}{cf.} 
\NewAbbr{ie}{i.e.,}

\NewAbbr{Whp}{W.h.p.}
\NewAbbr{whp}{w.h.p.}
\NewAbbr{Wlog}{W.l.o.g.}
\NewAbbr{wLOG}{w.l.o.g.}
\NewAbbr{wrt}{w.r.t.}

